EfficientLLM: Efficiency in Large Language Models

Large Language Models (LLMs) have driven significant progress, yet their growing parameter counts and context windows incur prohibitive compute, energy, and monetary costs. We introduce EfficientLLM, a novel benchmark and the first comprehensive empirical study evaluating efficiency techniques for LLMs at scale. Conducted on a production-class cluster (48xGH200, 8xH200 GPUs), our study systematically explores three key axes: (1) architecture pretraining (efficient attention variants: MQA, GQA, MLA, NSA; sparse Mixture-of-Experts (MoE)), (2) fine-tuning (parameter-efficient methods: LoRA, RSLoRA, DoRA), and (3) inference (quantization methods: int4, float16). We define six fine-grained metrics (Memory Utilization, Compute Utilization, Latency, Throughput, Energy Consumption, Compression Rate) to capture hardware saturation, latency-throughput balance, and carbon cost. Evaluating over 100 model-technique pairs (0.5B-72B parameters), we derive three core insights: (i) Efficiency involves quantifiable trade-offs: no single method is universally optimal; e.g., MoE reduces FLOPs and improves accuracy but increases VRAM by 40%, while int4 quantization cuts memory/energy by up to 3.9x at a 3-5% accuracy drop. (ii) Optima are task- and scale-dependent: MQA offers optimal memory-latency trade-offs for constrained devices, MLA achieves lowest perplexity for quality-critical tasks, and RSLoRA surpasses LoRA efficiency only beyond 14B parameters. (iii) Techniques generalize across modalities: we extend evaluations to Large Vision Models (Stable Diffusion 3.5, Wan 2.1) and Vision-Language Models (Qwen2.5-VL), confirming effective transferability. By open-sourcing datasets, evaluation pipelines, and leaderboards, EfficientLLM provides essential guidance for researchers and engineers navigating the efficiency-performance landscape of next-generation foundation models.

==> lora.tex <==
\noindent\textbf{Low-Rank Adaptation (LoRA) and Variants.}
A prominent PEFT strategy is Low-Rank Adaptation (LoRA) \cite{Hu2021LoRA}, which freezes the pre-trained weights \(W_0\) and introduces a trainable low-rank decomposition \(\Delta W = \alpha AB\) for task-specific updates, where \(A \in \mathbb{R}^{m \times r}\), \(B \in \mathbb{R}^{r \times n}\), and \(r \ll \min(m, n)\). The adapted weight is \(W = W_0 + \alpha AB\). This significantly reduces trainable parameters to \(r(m+n)\) and allows merging the update (\(\Delta W\)) into \(W_0\) after training, eliminating inference overhead \cite{Hu2021LoRA}.

Several recent methods build upon LoRA's foundation. LoRA+ \cite{Hayou2024LoRAplus} enhances training dynamics by using different learning rates for matrices \(A\) and \(B\), improving convergence speed and final performance without changing the parameterization. Rank-Stabilized LoRA (rsLoRA) \cite{Kalaj2023rsLoRA} modifies the scaling factor to \(\alpha = 1/\sqrt{r}\) (instead of the common \(\alpha/r\)), stabilizing training at higher ranks \(r\) and enabling better performance trade-offs. Weight-Decomposed LoRA (DoRA) \cite{Liu2024DoRA} reformulates the update by decomposing the weight matrix \(W\) into magnitude and direction components. It updates the direction using a LoRA-like structure applied to the normalized pre-trained directions \(D_0\), while learning a separate magnitude vector \(n\), resulting in \(W = (D_0 + AB)\,\mathrm{diag}(n)\). This separation often leads to improved performance by tackling magnitude and direction updates independently. Principal Singular Vectors Adaptation (PiSSA) \cite{Meng2024PiSSA} initializes the low-rank matrices \(A\) and \(B\) using the principal singular vectors and values derived from an SVD of the original weights \(W_0\). It trains \(W = AB + R\), where \(R\) is the frozen residual part of \(W_0\). This initialization aligns the adaptation with the most significant components of the pre-trained weights, often leading to faster convergence and better results compared to standard LoRA initialization. All these variants typically retain the benefit of zero inference overhead by merging the learned components post-training.
